Maximum Return on Investment for a Domestic Photovoltaic Installation

The rising energy prices in Europe and the urgent need to address global warming have sparked a significant increase in the installation of domestic photovoltaic systems to harness solar energy. However, since solar energy is available only during daytime hours and its availability varies daily, effectively shifting energy use becomes crucial. Whilst batteries can assist in storing excess energy, their high prices hinder their widespread adoption. In this study, we explore the importance of load to maximise return on investment. We propose an incremental approach to fitting load profiles into the production envelope, allowing for practical implementation. We compare different meter resolutions: 1 second, 5 minutes, 15 minutes, and 1 hour. Our analysis reveals that making real-time decisions (per second) leads to significant energy savings of 16\% compared to hourly decisions. Furthermore, we explore three types of device management strategies: ON/OFF management independent of PV production, ON/OFF management based on the current PV production, ON/OFF management based on both current and forecasted PV production, utilising an optimal fit algorithm. Through our study, we demonstrate that our implementation of the third approach outperforms a standard management approach, resulting in more than 17% cost savings. This study provides insights into the optimisation of load-shifting strategies in domestic photovoltaic installations, highlighting the importance of load control and the potential benefits in maximising the utilisation of solar energy while minimising energy costs and environmental impact.

==> background/background.tex <==
\chapter{Background}



==> design/design.tex <==
\chapter{Design}


==> evaluation/evaluation.tex <==
\chapter{Evaluation}

==> img3/characteristics.tex <==
\chapter{Load Characteristics, and Practical Considerations}

\section{Load Characteristics}
\subsection{Electric car} 
The majority of the electric-car charging is at constant power, e.g. cars come with a charger that allows for household plug charging (2.3 kW - 10 A at 230 V), or with a dedicated wallbox at a given power, oftentimes this is 7.36 kW or 11 kW (corresponding to 32A, 48 A, respectively with 230 V). However, charging at very high power (fast charging) reduces the battery longevity.

In France the average consumption is 50 minutes per person and per day, for an average distance of 36km \cite{art:1}. An electric car uses in average 0.161 kWh per km. Therefore in this study we assume the daily power requirement for the car is: 5.796 kWh. Furthermore, the average car battery has a capacity of 75 kWh [2].

Hence, given these information, we fix the charging time for the car at \textbf{2 hours 30 minutes}, because it is the charging time needed to satisfy the average consumption in France if we use a household plug charging of 2.3 kW. 


Practically, a longer trip with the car can be foreseen and may require manual intervention to boost the electric-car battery to maximum capacity. 

\subsection{Domestic hot water} 
There are a vast amount of water boilers deployed in homes today, and many use electricity as the primary source to heat hot water until the target temperature is reached (typically 60 °C). When the target temperature is reached the boiler's security system shuts heating OFF, and no electricity is consumed anymore beyond that point.

Per person and year, 800 kWh is the required energy for hot water in a household \cite{art:3}.
In France, there are an average of 2.19 people per household \cite{art:4}. So the estimated daily energy used in the household for hot water is 4.8 kWh.

Therefore, an average 2 kW water boiler requires 2.4 h of heating daily with 2 kWh electricity.
During the day, this form of water heating allows for load shifting as showers and hot water consumption is concentrated at the beginning and the end of the day.

In Summary:
\begin{itemize}
\item widely deployed
\item allows for ON/OFF and water storage allows for load-shifting
\item 2.4 hours at 2 kW every day
\end{itemize}

Usually, the typical pattern is full charge during 2 and half hours followed by brief intervals of full charging for a few minutes to maintain the water temperature at the desired level. In this study we only include the main big initial heating period of \textbf{2 hours 30 minutes} and neglect from the small periods.

\subsection{Pool pump} 
A pool pump is a device used to circulate and filter water in a swimming pool. It is responsible for pulling water from the pool, passing it through a filtration system to remove debris and contaminants, and then returning the clean water back to the pool.
The rule of thumb used for the running time of a pool pump that runs water through the filtration system is water temperature divided by 2 hours. 

So at 20 degrees water temperature, the pool pump is supposed to run for \textbf{10 hours} every day. Pool filtration and solar power go nicely hand-in-hand.

\section{Practical Considerations}

Our data from the 1st January 2023 to the 10th of April 2023 is from a 14.7 kWp PV installation in the South of France.

Network connectivity issues and outages resulted in a few missing data items every day. In a first step, we complete the input data to obtain data for every second of the day, 86400 items per day. Missing data is interpolated linearly, as shown in (\ref{fig:clean-data}). If there is one complete hour (or more) of missing data, we take the data of this time frame from the previous day (see \ref{fig:clean-data}). The time is in UTC.

\begin{figure}[H]
\hfill
\subfigure{\includegraphics[width=7cm]{img/graph15.png}}
\hfill
\subfigure{\includegraphics[width=7cm]{img/graph16.png}}
\hfill
\caption{}
\label{fig:clean-data}
\end{figure}


==> img3/forecast_load.tex <==
\chapter{The estimation of each load profile}

\section{Estimation of each device}
\label{sec:algo_load}
After having computed the PV forecasting, we need to estimate the consumption of a device. For perfect device management, the highest level of automation, and the avoidance of human errors, we use the automatically estimated device profiles to do the device and load management in the next chapter.

We want to estimate the consumption of a device, we have as input the time when the device is switched ON and the time when the device is switched OFF. Additionally, we have access to the global load of all devices during these periods. We assume the most common case, which is the presence of only one energy meter for the household. The problem can therefore be stated as: 
\begin{center}
    \textbf{Separating the energy consumed by one device from the sum of energy consumed by all devices.}
\end{center}

With the available ON/OFF timing information and the meter reading at all times, we search for the best estimate of the device consumption. We separate 2 cases:
\begin{itemize}
\item when the device switches ON, and
\item when the device switches OFF.
\end{itemize}
When the device switches ON, the load increases with a magnitude corresponding approximately to the consumption of the device. However, sometimes, the change is not instant, for example with the car (\ref{fig:firstON}). It often takes up to one minute after switching ON until the load becomes active and apparent on the meter reading.
\begin{figure}[H]
\hfill
\subfigure{\includegraphics[width=7cm]{img/graph5.png}}
\hfill
\subfigure{\includegraphics[width=7cm]{img/graph6.png}}
\hfill
\caption{}
\label{fig:firstON}
\end{figure}

When the device switches OFF, the load decreases with a magnitude corresponding approximately to the consumption of the device. The response is quicker after an OFF event than an ON event (see fig \ref{fig:firstON}).

To find the consumption of the device we do edge detection on the global load with a window of 10 seconds: 
we shift a window of 10 seconds over the load, and we save the absolute value of the difference of maximum and minimum inside the window as the device loads. To determine if it is an ON or an OFF event we verify the order, i.e. the minimum needs to be after the maximum for the ON event, while for the OFF event, it is the inverse. 

For an ON event, we search for the maximum load difference within a two-minute interval starting from the time when the device is switched ON (t to t + two minutes). Similarly, for an OFF event, we search for the maximum load difference within a one-minute interval starting from the time when the device is switched OFF (t to t + one minute). Furthermore, we apply exponential weighting to the window, meaning that an absolute difference measured between t and t + size of the window carries twice the weight of the absolute difference measured between t + size of the window and t + two times the size of the window. In summary, the consumption of a device is determined by the maximum weighted absolute difference, following the aforementioned conditions.

\section{Turbulent periods}
\label{sec:calm_periods}
A turbulent period is defined as a period that is not a "calm" period. A "calm" period is a 10 minutes period of load that has a standard deviation corresponding to the 10\% of the lowest standard deviations of all the 10 minutes periods of load of any given day.
As we know, devices are sometimes switched ON/OFF during turbulent periods and thus can lead to wrong results. 
In fact, two devices can be launched at the same time, and it will be very difficult to find the consumption of each device.  To enhance the accuracy of our device estimation, we considered the possibility of measuring the load change when activating a device during regular "calm" periods, aiming for the highest level of precision possible.
For n devices, we choose \begin{math} n\times(2+1)+1 \end{math} minutes to define a calm period. Three minutes per device (composed of two Minutes for the ON period, one Minute for the OFF period) and one Minute as a safety buffer for all devices. 

To forecast a calm period in a day, we compute all of the calm periods during the past 7 days and require that at least 5 of them overlap. The graph \ref{fig:overlapInterval} shows graphically points where calm periods overlap. 
\begin{figure}[H]
    \centering
    \includegraphics[width=5cm]{img/overlap_intervals.png}
    \caption{An example of overlapping intervals}
    \label{fig:overlapInterval}
\end{figure}
All these points forecasted the start of the calm periods for our current day. 
The graphs in Figure \ref{fig:pastDays} show that the two calm periods forecasted for the 26th of March 2023 start at 01:00 a.m. and 10:22 p.m., based on the data of the last 7 days (from the 19th of March 2023 to the 25th of March 2023). Therefore, on the 26th of March 2023, the measurement and device load estimation happens from 01:00 a.m. to 01:10 a.m. and from 10:22 p.m. to 10:32 p.m..

\begin{figure}[H]
\subfloat{\includegraphics[width = 5cm]{img/graph13.png}}
\subfloat{\includegraphics[width = 5cm]{img/graph12.png}} 
\subfloat{\includegraphics[width = 5cm]{img/graph11.png}} 
\subfloat{\includegraphics[width = 5cm]{img/graph10.png}} 
\subfloat{\includegraphics[width = 5cm]{img/graph9.png}}
\subfloat{\includegraphics[width = 5cm]{img/graph8.png}} 
\subfloat{\includegraphics[width = 5cm]{img/graph7.png}} 
\caption{The calm periods found from the 19th March 2023 to the 25th March 2023}
\label{fig:pastDays}
\end{figure}

Calm periods are often during times outside of the PV production window (most of the calm periods found are during the night), which means that we will need to pay electricity from the grid to test and to estimate the device loads. Devices might change, therefore device estimation is done on a continuous basis, always using the information from the past seven days. Once seven days of data have been, we have enough data to even avoid testing outside the PV production window. By taking the median on the data measured, we avoid the outliers caused during turbulent periods and maintain good results. The algorithm with the seven past days found the correct device consumption of each device for every day by taking the median of all the consumption measured for ON/OFF events without using the "calm" periods.

\section{Base load}
\label{sec:base_load}
Then we needed to find the “base load” to simulate the load of the devices that we do not have control onto, like the wash machine, the fridge, the lights etc. The “base load” is the load when all the ON/OFF controllable devices are OFF. 
To compute it, we just computed the median of all the loads measured when all the controllable devices (the car, the pool pump, and the domestic hot water) were OFF. 


==> img3/forecast_solar.tex <==
\chapter{The estimation of future solar production}

To estimate solar production, the starting point is the maximum possible production available for a given installation - the clearsky model.  
First, the real production data from every day of January 2023 is being visualized (\ref{fig:all-pv}).
\begin{figure}[H]
    \centering
    \includegraphics[width=15cm]{img/all_pv_sep.png}
    \caption{The real production data from every day of January 2023}
    \label{fig:all-pv}
\end{figure}
At first glance, the production curves resemble a normal distribution. We validate via the means squared error (MSE) how well the normal distribution approximates the maximum possible production (the clear sky model). If the normal distribution approximates well the clear sky model it will approximate also well the real production. We therefore start by approximating the real production data with a normal distribution to either validate or abandon the normal distribution as an approximation of the clear sky model.

We tried first to find the closest normal distribution for PV production of each given day. The normal distribution is defined by three parameters: the maximum, the mean, and the standard deviation. We selected the closest normal distribution for every production day in January 2023. 

To increase the speed of finding the closest distribution we optimized the search in the following way:
first, we selected the maximum value of the normal distribution in this range (in Watt):
\begin{equation} [max(pv) - 2000, max(pv) + 2000], \end{equation} second, we selected the mean of the normal distribution to be in the range from 8:20 AM to 4:40 PM, and third the standard deviation in the range of from 4000 seconds to 20000 seconds. Within this search space we chose the normal distribution with the smallest MSE. 
Even the best normal distribution didn’t well approximate the production data, as we see on the following graph. The graph \ref{fig:normdist} shows the day with the smallest MSE between normal distribution and production data (31th January 2023). The reader sees immediately that the start and the end of the PV production are far overestimated. The MSE is 362893.
\begin{figure}[H]
    \centering
    \includegraphics[width=8cm]{img/graph4.png}
    \caption{}
    \label{fig:normdist}
\end{figure}
We conclude that the normal distribution is not a good approximation of the production data, and therefore is also not a good approximation for the clear sky model. 

In the paper \cite{peratikou2022estimating} a method of estimating clear-sky PV electricity production without exogenous data is given. This article adopts a direct forecasting approach and thus, the proposed data-driven approach is dependent solely on historical time-series power output data from grid-connected without having to rely on the technical characteristics of the PV or on other energy or meteorological-related data, equipment, models, sky/satellite images, etc. 

Their method to estimate the clear sky is following:
\begin{enumerate}
\item The quantities that characterize the shape and the distribution of PV power output time-series at a given time are calculated first. The three criteria used are the mean value, the maximum value, and the standard deviation of the PV power output time series.
\item The calculated quantities were used as limits to the PV power output at each second. All the PV power output values outside the limits were excluded. Different limits were studied and tested in their study.
\item The predicted clear-sky signal is calculated by the resulting average of the PV power output time series within the limits for the corresponding month.
\end{enumerate}
The best method (with the smallest MSE) describes: 
\begin{equation}
upper limit = A + 1.5 SD 
\end{equation}\begin{equation}
lower limit = B. \\
\end{equation}
A is the mean value of the examined PV power output time series at a specific time. \\
SD is Standard Deviation of the examined PV power output time series at a specific time. \\
B is the average value of PV power output, excluding all points outside the upper limit and the lower limit band. \\
If we use the previous example of the 31st of January, with the use of the PV production of the last seven days (from the 24th of January 2023 to the 30th of January 2023), the algorithm outputs a predicted production for the 31th of January 2023 with a sufficient MSE of 68340, which is an 81\% decrease compared to the MSE of the normal distribution method (that knows the current PV production). Please see \ref{fig:forecast}.
\begin{figure}[H]
    \centering
    \includegraphics[width=8cm]{img/graph4_edi.png}
    \caption{}
    \label{fig:forecast}
\end{figure}
To measure the performance of the PV forecasting, we measured all the clear sky data we had: from the 8th of January (because we need 7 past days) to the 10th of April 2023. 
We computed the mean per second of the difference between the real PV production and the PV production forecasted for every day. The result is:
the forecast of the PV production overestimates the real PV production per second with a mean of \textbf{2.12\%}.
Please find the following graphs for the 10 best PV forecasts with \ref{fig:10best}.
\begin{figure}[H]
    \centering
    \includegraphics[width=15cm]{img/top10_forecasting.png}
    \caption{The 10 best PV forecasts from the 8th January to the 10th April 2023}
    \label{fig:10best}
\end{figure}


==> img3/optimal_fit.tex <==
\chapter{Optimal fitting of load profiles into the production envelope}
\section{Time Decision}
\label{sec:1}
We wanted to see the influence of the time frame for making decisions.
For that, we implemented a device management algorithm that works with decisions based on seconds, 5 minutes, 15 minutes, and 1 hour.

The algorithm works with the mode ‘adaptative’.

In the adaptive mode, we implement a dynamic threshold approach to optimize energy usage based on the PV production. A predefined threshold value is set, such as 4000 Ws, which represents the maximum power consumption allowed from the PV production.
To illustrate the adaptive mode, let's consider a scenario where the PV production is 3900 Ws at 1 pm, 4100 Ws at 2 pm, 4500 Ws at 3 pm, and 3800 Ws at 4 pm. At each time interval, we compare the PV production with the threshold value.
For instance, at 1 pm, the PV production of 3900 Ws is below the threshold of 4000 Ws, so no device will be activated during this period. However, at 2 pm, when the PV production reaches 4100 Ws, which exceeds the threshold, we initiate the activation of a controllable device.
Once the device is turned ON at 2 pm, it will consume the power from the PV production, in this case, 4000 Ws per second, for the duration of the activation period. In our example, the device will remain ON until 4 pm, utilizing the available 4000 Ws per second during this time frame.
Finally, at 4 pm, when the PV production drops below the threshold to 3800 Ws, we deactivate the device, turning it OFF as it can no longer operate at the desired power consumption level.

This adaptive mode allows us to dynamically adjust device activation based on the real-time PV production, ensuring optimal energy utilization within the constraints of the available power. By aligning device activation with higher PV production periods, we maximize the utilization of clean energy and minimize reliance on the grid or other energy sources.

The adaptative mode can make devices work in parallel and can combine multiple devices. For example, for every second, we can say that the car takes 3000 Ws, and the pool pump consumes 2000 Ws. Furthermore, most of the chargers are using constant charging.

To measure the difference between 15-minute, 15-minute and hour based decisions, I decided to launch an adaptive mode with a fixed threshold of 4000 Ws. 
The results are following \ref{fig:energyUsed}.

\begin{figure}[H]
    \centering
    \includegraphics[width=15cm]{img/Energy_used_from_PV.png}
    \caption{}
    \label{fig:energyUsed}
\end{figure}

\begin{table}[H]
\centering
\begin{tabular}{||c c c c||} 
 \hline
  & 5min & 15min & 1hour \\ [0.5ex] 
 \hline\hline
 mean & 98\% & 95\% & 84\% \\ 
 \hline
 median & 99\% & 97\% & 88\% \\
 \hline
 min & 91\% & 71\% & 28\% \\
 \hline
\end{tabular}
\end{table}

We notice that on the worst day of January 2023, an hour based decision is using \textbf{28\%} of the available production from PV.
Then, I wanted to see how much we will pay for energy from grid to satisfy the threshold (see \ref{fig:energyPaid}).

\begin{figure}[H]
    \centering
    \includegraphics[width=15cm]{img/Energy_paid_from_grid.png}
    \caption{}
    \label{fig:energyPaid}
\end{figure}

\begin{table}[H]
\centering
\begin{tabular}{||c c c c||} 
 \hline
  & 5min & 15min & 1hour \\ [0.5ex] 
 \hline\hline
 mean & 714.237kW & 1495.218kW & 7286.616kW \\ 
 \hline
 median & 581.408kW & 966.566kW & 6518.619kW \\
 \hline
 max & 3905.480kW & 4708.951kW & 17035.819kW \\
 \hline
\end{tabular}
\end{table}

We notice that on the worst day of January 2023, hour-based decisions will cause to pay 17035.819 kWs from grid. 1 kWh costs 0.2€ in France. 
17035.819 kWs equals approximately 4.73 kWh which makes approximately \textbf{0.95€} for the worst day of January 2023.

Over the first month period of real data, taking second-level decisions outperformed hourly decisions during 29 days. Over the whole period, we saved \textbf{16\%} of energy compared to hour-based decisions.

In the remainder of the report, we base our study purely on decisions by second.



\section{Optimal algorithm}
The problem now is to fit the load profile into the production envelope to maximize return on investment. First, money is saved by the consumption of cheap energy. Second, money is gained by selling excess capacity to the electricity provider.

Currently, the price to buy 1 kWh in France is 0.2€, and the price to sell 1 kWh to the electricity provider is 0.13€. Furthermore, we can not sell more than 6 kW per second.

With this information, we deduct the following constants for day \begin{math}j\end{math}:
\begin{align*} 
    E_{max,sell} &= 6 kWs  \\
    C_{e,sell} &= 0.13  EUR/kWh  \\
    C_{e,buy} &= 0.2  EUR/kWh 
\end{align*}
We name the 2 following functions for the load and the PV production: 
\begin{itemize}
\item P(j, t): "The PV production in kW for day \begin{math}j\end{math} at time \begin{math}t\end{math} seconds" 
\item L(j, t): "The load in kW for day \begin{math}j\end{math} at time \begin{math}t\end{math} seconds" \\
\end{itemize}
We therefore have one combined optimization function of money that comes from saving and selling:
\\
\[
M(j) = S(j) - B(j)
\]
\begin{center}
which is the money in € for day \begin{math}j\end{math}.
\end{center}
\\
\[
S(j) =  \sum_{t=0}^{86399} min(E_{max,sell}, max(P(j, t) + L(j, t), 0))\times  \frac{C_{e,sell}}{3600s} 
\]
\begin{center}
which is the money in € we gain by selling energy on day \begin{math}j\end{math}. 
\end{center}
\\
\[
B(j) = \sum_{t=0}^{86399} max(0, -P(j, t) - L(j, t))\times  \frac{C_{e,buy}}{3600s} 
\]
\begin{center}
which is the money in € spent by buying energy on day \begin{math}j\end{math}.
\end{center}
\\

Our first idea was to work with basic conditions on thresholds (adaptative mode described in section \ref{sec:1}), for example if the PV production deducted by the existing loads is greater than the consumption device \begin{math}i\end{math} at time \begin{math}t\end{math}, then we can switch device \begin{math}i\end{math} ON. If the PV production deducted by the existing loads is less than the consumption device \begin{math}i\end{math} at time \begin{math}t\end{math}, then we switch device \begin{math}i\end{math} OFF.

The problem with this algorithm is that it does not maximize electricity sales on sunny days, as sales have an upper bound. In fact, because it will turn on all the devices linearly with the beginning of the PV production, and then at the peak of the PV production, we can only sell 6 kW per second, so we will lose some PV production.

Then, we tried a different approach given the PV forecasting by maximizing the function \begin{math}M\end{math}. The idea is to define the loads of each device as a rectangle. In fact, the height of the rectangle is the consumption of the device, and its length is the time the device needs to be on. We then place the rectangle of each device by the reverse order of length (rectangle with maximum length is placed first) to maximize the function \begin{math}M\end{math}, shown in Figure \ref{fig:rectangles}.

\begin{figure}[H]
    \centering
    \includegraphics[width=8cm]{img/graph14.png}
    \caption{}
    \label{fig:rectangles}
\end{figure}

Then, when we have our forecasting of when our device $i$ should start: ($\mathbf{T}_{device, ON_i}$), and when our device $i$ should end: ($\mathbf{T}_{device, OFF_i}$). We define algorithm \ref{alg:cap} to be in concordance with the current production. 
This algorithm will thus adapt our original rectangles by creating different rectangles of different lengths (but with the same height) to adapt to the current production if the forecasted production is different (\ref{fig:real}). 





\begin{figure}[H]
    \centering
    \includegraphics[width=15cm]{img/Optimal_energy.png}
    \caption{}
    \label{fig:real}
\end{figure}

\section{Results}
\label{sec:results}

To assess the efficacy of our device management algorithm, I conducted three simulations spanning from January 8th (considering the need for seven previous days) to April 10th, 2023, using 9 kWp solar panels.

The first simulation employed the smart device management algorithm described in this report, prioritizing three devices in the following order: the pool pump, domestic hot water, and the car. A device A is considered to have higher priority than device B if, under the same conditions for activation, device A is switched on first. Similarly, if given the same conditions for deactivation, device A is switched off last.

In the second simulation, we scheduled the activation of the pool pump at 10 am, domestic hot water at 7 pm, and the pool device at 12 pm each day. Each device was switched off after running for the same duration as in the first simulation. We chose these specific starting times based on our analysis of load data before the installation of the solar panels. This device management strategy is referred to as "bruteforce."

The third simulation utilized the adaptive mode outlined in section \ref{sec:1}. In this mode, the threshold for each device's activation is based on its consumption level. It should be noted that the car was installed on March the 25th, and, therefore, its consumption did not need to be managed before that date.






\subsection{Comparison of Smart and Bruteforce management simulation}
The simulation results presented in Figure \ref{fig:bruteforce} depict that the bruteforce device management algorithm consistently achieves higher daily sales compared to the smart management algorithm. This disparity can be attributed to the fact that the smart management algorithm prioritizes maximizing the consumption of solar production over selling it, considering that the cost of purchasing energy exceeds the price of selling energy.

The concept of maximizing the utilization of PV production is further substantiated by Figure \ref{fig:bruteforce}, which demonstrates that the bruteforce device management algorithm incurs greater daily purchases compared to the smart management algorithm.

\begin{figure}[H]
\hfill
\subfigure{\includegraphics[width=7cm]{img/Sales[EUR] Smart Management and Sales[EUR] Bruteforce Management .png}}
\hfill
\subfigure{\includegraphics[width=7cm]{img/Purchase[EUR] Smart Management and Purchase[EUR] Bruteforce Management.png}}
\hfill
\caption{}
\label{fig:bruteforce}
\end{figure}

To assess the overall performance of each device management approach, we compute the daily balance by summing the sales and purchases. Figure \ref{fig:diff_bruteforce} displays the cumulative balance for each management algorithm throughout the given period. Notably, the cumulative balance for the smart management algorithm consistently surpasses that of the bruteforce management algorithm.

Furthermore, by analyzing the statistics for the daily balance of each device management approach, we find that, on average, our algorithm achieves savings of approximately \textbf{0.43€} per day, which translates to approximately \textbf{157€} per year. Consequently, our algorithm yields \textbf{17.3\%} higher cost savings compared to the bruteforce approach.

However, it is important to note that the difference between the cumulative balance of the bruteforce management and the smart management varies over time, as depicted in Figure \ref{fig:diff_bruteforce}, indicating a non-linear relationship.

In summary, our simulation-based comparison demonstrates the superior performance of the smart management algorithm in optimizing energy consumption and financial savings. By maximizing the utilization of PV production, our algorithm consistently outperforms the bruteforce approach, resulting in significant cost reductions.

\begin{figure}[H]
\hfill
\subfigure{\includegraphics[width=7cm]{img/Cumulative Balance[EUR] Smart Management and Cumulative Balance[EUR] Bruteforce Management.png}}
\hfill
\subfigure{\includegraphics[width=7cm]{img/Difference between Cumulative Balance[EUR] Bruteforce Management and Cumulative Balance[EUR] Smart Management.png}}
\hfill
\caption{}
\label{fig:diff_bruteforce}
\end{figure}

\subsection{Comparison of Smart and Adaptative management simulation}
Next, we proceed to compare the results of the first simulation (Smart management) with the third simulation (Adaptive management). Similar to the previous comparison, the outcomes presented in Figure \ref{fig:constant} demonstrate that the Adaptive device management algorithm consistently achieves higher daily sales compared to the Smart management algorithm. This can be attributed to the fact that the Smart management algorithm possesses an optimal solution for maximizing PV consumption compared to the Adaptive management algorithm.

The notion of maximizing the utilization of PV production is further validated by Figure \ref{fig:constant}, which illustrates that the daily purchases made by the Adaptive device management algorithm surpass those of the Smart management algorithm.

\begin{figure}[H]
\hfill
\subfigure{\includegraphics[width=7cm]{img/Sales[EUR] Smart Management and Sales[EUR] Adaptive Management.png}}
\hfill
\subfigure{\includegraphics[width=7cm]{img/Purchase[EUR] Smart Management and Purchase[EUR] Adaptive Management.png}}
\hfill
\caption{}
\label{fig:constant}
\end{figure}
As in the previous comparison, we calculate the daily balance by summing the sales and purchases, and the results are shown in Figure \ref{fig:diff_constant}. Notably, the cumulative balance for the Smart management algorithm consistently surpasses that of the Adaptive management algorithm.

Moreover, by analyzing the statistics for the daily balance of each device management approach, we observe an average savings of approximately \textbf{0.07€} per day, equivalent to approximately \textbf{26€} per year. Consequently, our algorithm achieves cost savings that are \textbf{2.8\%} higher than those of the Adaptive management algorithm.

The difference in cumulative balances between the two device management algorithms is illustrated in Figure \ref{fig:diff_constant}.

In summary, our comparative simulation of Smart and Adaptive device management algorithms demonstrates that the Smart management algorithm outperforms the Adaptive management algorithm in maximizing energy consumption and achieving financial savings. By optimizing PV utilization, our algorithm consistently yields higher sales and cumulative balance, resulting in significant cost reductions compared to the Adaptive management approach.


\begin{figure}[H]
\hfill
\subfigure{\includegraphics[width=7cm]{img/Cumulative Balance[EUR] Smart Management and Cumulative Balance[EUR] Adaptive Management.png}}
\hfill
\subfigure{\includegraphics[width=7cm]{img/Difference between Cumulative Balance[EUR] Adaptive Management and Cumulative Balance[EUR] Smart Management.png}}
\hfill
\caption{}
\label{fig:diff_constant}
\end{figure}


==> implementation/implementation.tex <==
\chapter{Implementation}
